Streaming, Memory Limited Algorithms for Community Detection

In this paper, we consider sparse networks consisting of a finite number of non-overlapping communities, i.e. disjoint clusters, so that there is higher density within clusters than across clusters. Both the intra- and inter-cluster edge densities vanish when the size of the graph grows large, making the cluster reconstruction problem nosier and hence difficult to solve. We are interested in scenarios where the network size is very large, so that the adjacency matrix of the graph is hard to manipulate and store. The data stream model in which columns of the adjacency matrix are revealed sequentially constitutes a natural framework in this setting. For this model, we develop two novel clustering algorithms that extract the clusters asymptotically accurately. The first algorithm is {\it offline}, as it needs to store and keep the assignments of nodes to clusters, and requires a memory that scales linearly with the network size. The second algorithm is {\it online}, as it may classify a node when the corresponding column is revealed and then discard this information. This algorithm requires a memory growing sub-linearly with the network size. To construct these efficient streaming memory-limited clustering algorithms, we first address the problem of clustering with partial information, where only a small proportion of the columns of the adjacency matrix is observed and develop, for this setting, a new spectral algorithm which is of independent interest.

==> proofs_before.tex <==



\section{Proofs}
In this section, we give proof of the following theorems.

\begin{theorem}\label{th:1} 
Assume that $\sqrt{\gamma}f(n)=o(1)$. Then under any clustering algorithm $\pi$, the expected proportion of misclassified green nodes tends to 1/2 as $n$ grows large, i.e., $\lim_{n\to\infty}\mathbb{E}[\varepsilon^\pi(n^{(g)})]=1/2$.
\end{theorem}

\begin{theorem}\label{th:2}
(i) If there exists a clustering algorithm that classifies the green nodes asymptotically accurately, then we have: $\sqrt{\gamma}f(n)=\omega(1)$.\\
(ii) If there exists an asymptotically accurate clustering algorithm (i.e., classifying all nodes asymptotically accurately), then we have: ${\gamma}f(n)=\omega(1)$.
\end{theorem}
\setcounter{theorem}{3}
\begin{theorem}\label{th:3}
When $\sqrt{\gamma} f(n) = \omega(1)$,
Algorithm~1 classifies the green nodes asymptotically accurately.
\end{theorem}

\begin{theorem} When $\gamma f(n) = \omega(1)$, combining Algorithms 1 and 2 yields an asymptotically accurate clustering algorithm.
\label{thm:clust-algor-red}
\end{theorem}


\begin{theorem} Assume that $h(n)=\omega({\log(n)\over \min\{ f(n), n^{1/3} \}})$  and $T=\omega({n\over
    \min\{ f(n), n^{1/3} \}})$. Then with $M = \Theta(n h(n) + n)$
  bits, Algorithm 3, with block size $B={h(n)n\over \min\{ f(n), n^{1/3} \}\log(n)}$ and acquiring the $T$ first columns of $A$, outputs clusters $\hat{V}_1,\ldots,\hat{V}_K$ such that with high probability, there exists a permutation $\sigma$ of $\{1,\ldots,K\}$ such that: 
$$
\frac{1}{n} \left|\bigcup_{1\le k \le K} \hat{V}_k \setminus V_{\sigma(k)}
\right| = O\left( \exp(-T{\min\{ f(n), n^{1/3} \}\over n}) \right). 
$$
\label{thm:streaming-with-green}
\end{theorem}


For the proofs, we denote by $\lambda_i (X)$ the $i$-th largest
singular value of matrix $X$. 

\subsection{Proof of Theorem~\ref{th:1} }
\iffalse
\begin{theorem}
Assume that $\sqrt{\gamma}f(n) = o(1)$. Then for any clustering
algorithm $\pi$, the expected proportion of misclassified green nodes is
$1/2$, i.e.
\begin{eqnarray*}
\lim_{n\to \infty}\mathbb{E}[\epsilon^\pi(n^{(g)})] = 1/2.
\end{eqnarray*}
\end{theorem}
\fi

For any $k>0$ and any two vectors $x,y\in\{1,-1\}^k$, we denote by
$d_H(x,y) = \sum_{i=1}^k 1(x_i\neq y_i)$ the Hamming distance and
define
\begin{eqnarray*}
d(x,y) = \frac{1}{k} \min\{d_H(x,y), d_H(x,-y)\}.
\end{eqnarray*}

For an estimate $\hat{\sigma}^{(g)}$ of $\sigma^{(g)}$, the quantity
$d(\hat{\sigma}^{(g)},\sigma^{(g)})$ is exactly the fraction of
misclassified green nodes. Hence if estimate $\hat{\sigma}^{(g)}$ is
obtained from algorithm $\pi$, we have
$\epsilon^\pi(n^{(g)})=d(\hat{\sigma}^{(g)},\sigma^{(g)})$.


Note that $d(\hat{\sigma}^{(g)},\sigma^{(g)})\leq 1/2$. If
$\hat{\sigma}^{(g)}$ is a random guess, i.e. for each $v\in V^{(g)}$,
  $\hat{\sigma}^{(g)}_v$ is equal to $1$ or $-1$ with probability
  $1/2$ independently of the rest, then for any $\alpha<1/2$, as soon as $n^{(g)}\to \infty$, we
  have by the weak law of large numbers,
$\mathbb{P}(d(\hat{\sigma}^{(g)},\sigma^{(g)})>\alpha) \to 1$.
\iffalse
Hence, we define for $\alpha<1/2$,
\begin{eqnarray*}
\delta(\alpha) = 1 -\inf_{\hat{\sigma}^{(g)}}
\mathbb{P}(d(\hat{\sigma}^{(g)},\sigma^{(g)})>\alpha)\geq 0,
\end{eqnarray*}
where the infimum ranges over all estimates $\hat{\sigma}^{(g)}$ that
are mesurable function of the data $A$.
There exists a clustering algorithm asymptotically better than random guess
if $\delta(\alpha)$ does not tend to $0$.
\fi

\begin{lemma}
For any $\alpha<1/2$ and estimate $\hat{\sigma}^{(g)}$, we have as $m\to \infty$
\begin{eqnarray*}
\mathbb{P}(d(\hat{\sigma}^{(g)},\sigma^{(g)})>\alpha) \geq 1-\frac{n^{(g)}-H(\sigma^{(g)}|A)}{n^{(g)}(1-H(\alpha))}+o(1),
\end{eqnarray*}
where $H(\alpha) = -\alpha\log \alpha -(1-\alpha)\log(1-\alpha)$ and
$H(\sigma^{(g)}|A)$ is the conditional entropy of $\sigma^{(g)}$
knowing $A$.
\end{lemma}
{\it Proof:} We define the event
$E=\{d(\hat{\sigma}^{(g)},\sigma^{(g)})>\alpha\}$ and $P_e$ its probability.
We have
\begin{eqnarray*}
H(E,\sigma^{(g)}|\hat{\sigma}^{(g)}) &=&
H(\sigma^{(g)}|\hat{\sigma}^{(g)})+\underbrace{H(E|\sigma^{(g)},\hat{\sigma}^{(g)})}_{0}\\
&=& H(E|\hat{\sigma}^{(g)})+H(\sigma^{(g)}|E,\hat{\sigma}^{(g)})\\
&\leq& H(P_e) + P_e\log{n^{(g)} \choose n^{(g)}/2} +(1-P_e)(n^{(g)}H(\alpha)+\log n^{(g)}),
\end{eqnarray*}
where the last inequality follows from $H(E|\hat{\sigma}^{(g)})\leq
H(E) = H(P_e)$ and the fact that
\begin{eqnarray*}
|\{\sigma^{(g)}, d(\sigma^{(g)}, \hat{\sigma}^{(g)}) \leq
\alpha\}|=\sum_{i=0}^{\alpha n^{(g)}} {n^{(g)}\choose i}\leq (n^{(g)}\alpha+1){n^{(g)}\choose
\alpha n^{(g)}}\leq n^{(g)}2^{n^{(g)}H(\alpha)}.
\end{eqnarray*}
Using $H(P_e)\leq 1$ and that ${n^{(g)}\choose n^{(g)}/2} \leq 2^{n^{(g)}}$ for
sufficiently large $n^{(g)}$, we get
\begin{eqnarray*}
P_e \geq \frac{H(\sigma^{(g)}|\hat{\sigma}^{(g)})-1-n^{(g)} H(\alpha)-\log
  n^{(g)}}{n^{(g)}(1-H(\alpha))-\log n^{(g)}}.
\end{eqnarray*}
The claim follows from the data processing inequality which ensures
$H(\sigma^{(g)}|\hat{\sigma}^{(g)})\geq H(\sigma^{(g)}|A)$.

We have
\begin{eqnarray*}
H(\sigma^{(g)}|A) = H(\sigma^{(g)})-H(A) +H(A|\sigma^{(g)}).
\end{eqnarray*}
The first term is simple to compute: $H(\sigma^{(g)}) = \log {n^{(g)}\choose
  n^{(g)}/2} \geq n^{(g)}-\frac{1}{2}\log 2n^{(g)}$ and for the second term, we have
\begin{lemma}\label{lem:MI}
As $n^{(g)}\to \infty$, we have:
\begin{eqnarray*}
H(A) -H(A|\sigma^{(g)}) \leq o(n^{(g)})+O(n^{(g)}\gamma f(n)^2).
\end{eqnarray*}
\end{lemma}
Before proving it, we show how to conclude the proof of Theorem
\ref{th:1}.
As soon as $n^{(g)}\to \infty$, combining the two lemmas, we see
that for any $\alpha<1/2$ and any estimate $\hat{\sigma}^{(g)}$,
\begin{eqnarray*}
\mathbb{P}(d(\hat{\sigma}^{(g)},\sigma^{(g)})>\alpha) = 1+O(\gamma f(n)^2).
\end{eqnarray*}
But we have
\begin{eqnarray*}
\mathbb{E}[\epsilon^\pi(n^{(g)})]\geq \alpha \mathbb{P}(d(\hat{\sigma}^{(g)},\sigma^{(g)})>\alpha),
\end{eqnarray*}
and since $\alpha$ can be chosen as close to $1/2$ as desired, the
result follows.


{\it Proof of Lemma \ref{lem:MI}:} Thanks to independence, we have
\begin{eqnarray*}
H(A) - H(A | \sigma^{(g)}) 
& = & H(A^{(g)}) - H(A^{(g)} | \sigma^{(g)})+H(A^{(r)}) - H(A^{(r)} |\sigma^{(g)})
\end{eqnarray*}
We first deal with the first term $H(A^{(g)}) - H(A^{(g)} |
\sigma^{(g)})$. By the concavity of $p\mapsto H(p)$, we have
$H(A^{(g)})\leq {n^{(g)}\choose 2} H\left(\frac{p+q}{2} \right)$ and $H(A^{(g)} | \sigma^{(g)}) = 2{n^{(g)}/2
  \choose 2} H(p) + (\frac{n^{(g)}}{2})^2 H(q)$.
Hence, we get
\begin{align*}
H(A^{(g)}) - H(A^{(g)} | \sigma^{(g)}) \le & {n^{(g)} \choose 2}
H(\frac{p+q}{2}) - 2{n^{(g)}/2
  \choose 2} H(p) - (\frac{n^{(g)}}{2})^2 H(q) \cr
=&\frac{(n^{(g)})^2}{4}\left( 2H(\frac{p+q}{2}) - H(p) - H(q) \right) + o(n^{(g)})
\cr
=&\frac{(n^{(g)})^2}{4} \left(p\log \frac{2p}{p+q} +q\log \frac{2q}{p+q}\right) \cr &+
\frac{(n^{(g)})^2}{4}\left((1-p)\log\frac{2-2p}{2-p-q}+(1-q)\log\frac{2-2q}{2-p-q}
\right)+ o(n^{(g)})\cr
\le&\frac{(n^{(g)})^2}{4} \left( \frac{(p-q)^2}{p+q} + \frac{(p-q)^2}{2-p-q}
\right) + o(n^{(g)})\\
=& o(n^{(g)}) + o(n^{(g)}\gamma f(n)).
\end{align*}

We denote by $A^{(r)}_v$ the row vector of
$A^{(r)}$ corresponding to $v\in V^{(r)}$.
For the second term,  by independence we have
\begin{eqnarray*}
H(A^{(r)}) - H(A^{(r)} |\sigma^{(g)}) = (n-n^{(g)})\big( H(A_v^{(r)}) -
H(A_v^{(r)} | \sigma^{(g)})\big).
\end{eqnarray*}
For a vector $x\in \{-1,1\}^{V^{(g)}}$ and $\sigma^{(g)}$, we define
$|x|^+ = \sum_{v\in V^{(g)}, \:\sigma^{(g)}_v=1}x_v$, $|x|^- =
\sum_{v\in V^{(g)}, \:\sigma^{(g)}_v=-1}x_v$ and $|x|=|x|^++|x|^-$.
For a given $\sigma^{(g)}$, we have
$$\mathbb{P}[ A_v^{(r)} = x | \sigma^{(g)}] = \zeta ( |x|^+ , |x|^- ) ,$$
where
$$\zeta (i,j) = \frac{((\frac{p}{1-p})^{i}(\frac{q}{1-q})^{j}+(\frac{p}{1-p})^{j}(\frac{q}{1-q})^{i})(1-p)^{\frac{m}{2}}(1-q)^{\frac{m}{2}}}{2} .$$
Since $\sigma^{(g)}$ is uniformly distributed,
\begin{align*}
\mathbb{P}[ A_v^{(g)} = x ] =& {n^{(g)} \choose n^{(g)}/2}^{-1}
\sum_{\sigma^{(g)}:\sum_{v\in V^{(g)}}\sigma_v^{(g)}=0} \mathbb{P}[
A_v^{(g)} = x | \sigma^{(g)}] \cr
=& {n^{(g)} \choose n^{(g)}/2}^{-1}  \sum_{i=0}^{|x|}{|x| \choose
  i}{n^{(g)}-|x| \choose n^{(g)}/2-i} \zeta(i,|x|-i)  = \eta(|x|),
\end{align*}
where
$$\eta(k) = \frac{\sum_{ i=0}^{k} {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose k-i}
\zeta(i,k-i)}{\sum_{ i=0}^{k} {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose k-i}} .$$
Since $\eta(0) = \zeta(0,0)$, $\eta(1) = \zeta(1,0)=\zeta(0,1)$, and
${n^{(g)} \choose k} \eta(k) = \sum_{i=0}^{ k} {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose k-i}
\zeta(i,k-i),$
\begin{align*}
&H(A_v^{(r)}) - H( A_v^{(r)} | \sigma^{(g)} ) \cr 
&=-\sum_{k=0}^{ n^{(g)} }  {n^{(g)} \choose k}
\eta(k) \log \eta(k)   +\sum_{i=0}^{n^{(g)}/2}\sum_{j=0}^{ n^{(g)}/2 }  {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose j}
\zeta(i,j) \log \zeta(i,j)  \cr
 &= \sum_{i=0}^{n^{(g)}/2}\sum_{j=0}^{ n^{(g)}/2 } {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose j}
\zeta(i,j) \log \frac{\zeta(i,j)}{\eta(i+j)} \cr
& =\sum_{k=2}^{n^{(g)}} \sum_{i=0}^{k} 1_{i \le n^{(g)}/2} 1_{k-i \le n^{(g)}/2}  {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose k-i}
\zeta(i,k-i) \log \frac{\zeta(i,k-i)}{\eta(k)} \cr
&\le \sum_{k=2}^{n^{(g)}} \sum_{i=0}^{k} 1_{i \le n^{(g)}/2} 1_{k-i \le n^{(g)}/2}  {n^{(g)}/2 \choose i}{n^{(g)}/2 \choose k-i}
\zeta(i,k-i) k \log (\frac{p}{q}) \cr 
&\le \sum_{2\le k \le n^{(g)}} (n^{(g)}p)^k k \log (\frac{a}{b}) \cr
& = O((n^{(g)})^2 p^2 ),\end{align*}
where the last equality stems from $n^{(g)}p = o(1)$.
Thus,
$$(n-m)\big( H(A_v^{(r)}) - H(A_v^{(r)} | \sigma^{(g)})\big) = O(n(n^{(g)})^2
p^2 )  = O(n^{(g)} \frac{n^{(g)}}{n} f(n)^2 ) = O(n^{(g)}\gamma f(n)^2),$$ and the lemma
follows since $f(n)\geq 1$ so that $f(n)^2\geq f(n)$.





\subsection{Proof of Theorem~\ref{th:2}}

\iffalse
Consider that $m = \Theta(n)$ ($\gamma = \Theta(1)$). In Theorem~\ref{thm:clugreen},  $f(n) = \omega(1)$ is a 
necessary condition for accurate detection. From this, we conclude that $\sqrt{\gamma}
f(n) = \omega(1)$ is a necessary condition since $\gamma =
\Theta(1)$.
\fi

In the remaining proofs, we use $m$ instead of $n^{(g)}$ to denote the
number of green nodes. We first consider case (i) with $\gamma=\Theta(1)$. In this case, a
necessary condition for the existence of an asymptotically accurate
clustering algorithm is that the fraction of green nodes outside the
largest connected component of the observed graph vanishes as $n\to
\infty$. This condition imposes that $f(n)\to \infty$.

We now consider case (i) with $m = o(n)$, i.e. $\gamma
= o(1)$. Denote
by $\Phi$ the true hidden partition $(V^{(g)}_1 , V^{(g)}_2)$ for
green nodes. Let $\mathbb{P}_{\Phi}$ be the probability measure
capturing the randomness in the observations assuming that the network
structure is described by $\Phi$. We also introduce a slightly
different structure $\Psi$. The latter is described by clusters
$V'^{(g)}_1 =V^{(g)}_1 \cup \{v_2 \}\setminus \{ v_1 \}$,
$V'^{(g)}_2=V^{(g)}_2 \cup \{v_1 \} \setminus \{ v_2 \}$ with
arbitrary selected $v_1\in V^{(g)}_1$ and $v_2 \in V^{(g)}_2$.

Let $\pi\in \Pi'$ denote a clustering algorithm for green nodes with
output $(\hat{V}^{(g)}_1, \hat{V}^{(g)}_2)$, and let $\mathcal{E} =
\hat{V}^{(g)}_1 \bigtriangleup  V^{(g)}_1$ be the set
of misclassified nodes under $\pi$. Note that in general in our
proofs, we always assume without loss of generality that $|
\hat{V}^{(g)}_1 \bigtriangleup V^{(g)}_1 | \le |\hat{V}^{(g)}_1 \bigtriangleup V^{(g)}_{2}|$, so that the set of misclassified nodes is really
$\mathcal{E}$. Further define $\mathcal{B}=\{ v_1 \in \hat{V}^{(g)}_1\}$ as the set of events where node $v_1$ is
correctly classified. We have $\varepsilon (m) = |\mathcal{E}|/m$.

Let $x_{i,j}$ be equal to one if there is an edge between nodes $i$
and $j$ and zero otherwise.%denote the label observed on node pair $(i,j)$. 
With a slight abuse of notation, we define the boolean functions $p(\cdot)$ and
$q(\cdot)$ as follows: $p(1) = af(n)/n=p$, $q(1)=bf(n)/n=q$ and
$p(0)=1-p(1)$, $q(0)=1-q(1)$. We introduce $L$ (a quantity that resembles the log-likelihood ratio
between $\mathbb{P}_\Phi$ and $\mathbb{P}_{\Psi}$) as:

\begin{align*}
L =& \sum_{i \in V_1'^{(g)}}\log \frac{q(x_{i,v_1})p(x_{i,v_2})}{p(x_{i,v_1})q(x_{i,v_2})} + 
\sum_{i \in V_2'^{(g)}}\log
\frac{p(x_{i,v_1})q(x_{i,v_2})}{q(x_{i,v_1})p(x_{i,v_2})} \cr
&+ \sum_{v \in V^{(r)}} \log \frac{\prod_{i \in
    V_1'^{(g)}}p(x_{v,i})\prod_{i \in V_2'^{(g)}}q(x_{v,i}) + \prod_{i \in V_1'^{(g)}}q(x_{v,i})\prod_{i \in V_2'^{(g)}}p(x_{v,i})}{\prod_{i \in
    V_1^{(g)}}p(x_{v,i})\prod_{i \in V_2^{(g)}}q(x_{v,i}) + \prod_{i \in V_1^{(g)}}q(x_{v,i})\prod_{i \in V_2^{(g)}}p(x_{v,i})},
\end{align*}
In what follows, we establish a relationship between $\mathbb{E} [\varepsilon (m) ]$ and $L$. For any function $g(m)$, 
\begin{eqnarray} 
\mathbb{P}_{\Psi} \{ L \le  g(m) \}& =& \mathbb{P}_{\Psi} \{ L \le g(m) , \bar{\mathcal{B}} \} + \mathbb{P}_{\Psi} \{ L \le g(m) , \mathcal{B} \}. 
\end{eqnarray}
We have: 
\begin{eqnarray}\mathbb{P}_{\Psi} \{ L \le  g(m) , \bar{\mathcal{B}}\} &= &
  \int_{\{ L \le  g(m) , \bar{\mathcal{B}}\}} d\mathbb{P}_{\Psi} \cr
&= & \int_{\{ L \le  g(m) , \bar{\mathcal{B}}\}} \prod_{i \in
  V_1'}\frac{\nu(x_{i, v_1})\nu(x_{i,v_2})}{p(x_{i,v_1})q(x_{i,v_2})}
\prod_{i \in V_2'}\frac{\nu(x_{i,v_1})\nu(x_{i,v_2})}{q(x_{i, v_1})p(x_{i,v_2})} d\mathbb{P}_{\Phi} \cr
&\le & \exp (g(m))\mathbb{P}_{\Phi} \{ L \le  g(m) , \bar{\mathcal{B}}\}~ \le ~ \exp (g(m))\mathbb{P}_{\Phi} \{ \bar{\mathcal{B}}\}\cr
&\le &2\exp (g(m))\mathbb{E}_{\Phi} [ \varepsilon (m)], \label{eq:chofm-1}
\end{eqnarray}
where the last inequality comes from the fact that,
\begin{eqnarray*}\mathbb{P}_{\Phi} \{ \mathcal{B} \} &\ge& 1- \mathbb{P}_{\Phi} \{ v_1 \notin
\hat{V}^{(g)}_1 \} \ge 1-2 \mathbb{E}_{\Phi}[ \varepsilon(n) ]. \end{eqnarray*}
We also have: 
\begin{equation}\mathbb{P}_{\Psi} \{ L \le  g(m) , \mathcal{B} \} \le
  \mathbb{P}_{\Psi} \{  \mathcal{B} \} \le
2 \mathbb{E}_{\Psi}[ \varepsilon(m) ]. \label{eq:chofm-2}
\end{equation} 
By \eqref{eq:chofm-1} and \eqref{eq:chofm-2}
$$\mathbb{P}_{\Psi} \{ L \le  g(n) \} \le 2\mathbb{E}_{\Phi}[\varepsilon(n) ]\exp(g(n)) +
2 \mathbb{E}_{\Psi}[ \varepsilon(n) ]. $$
Since  $\mathbb{E}_{\Phi}[\varepsilon(n) ]
=\mathbb{E}_{\Psi}[\varepsilon(n) ] =\mathbb{E} [\varepsilon(n) ]$ and
$\mathbb{E} [\varepsilon(n) ] = o(1)$,
 choosing $g(m) = \log
\left( \frac{1 }{8 \mathbb{E} [ \varepsilon(m) ]} \right)$, we obtain:\begin{equation}
 \lim\inf_{m \rightarrow \infty}\mathbb{P}_{\Psi} \{ L \ge  \log \left( \frac{1}{8 \mathbb{E} [ \varepsilon(m) ]} \right) \} > \frac{1}{2}. 
\end{equation}
By Chebyshev's inequality, $\mathbb{P}_{\Psi} \{ L \ge
\mathbb{E}_{\Psi}[L] + 2\sigma_{\Psi}[L] \} \le
\frac{1}{4}$. Therefore, to be valid the above inequality,
\begin{equation}
\mathbb{E}_{\Psi}[L] + 2\sigma_{\Psi}[L] \ge \log \left(\frac{1}{8 \mathbb{E} [ \varepsilon(m) ]} \right),
\end{equation}
which implies that $\mathbb{E}_{\Psi}[L] + 2\sigma_{\Psi}[L] =
\omega(1)$ since $\mathbb{E} [ \varepsilon(m) ] = o(1)$.

We define $KL(p,q)=p\log(p/q)+(1-p)\log((1-p)/(1-q))$.
From the definition of $L$, we can easily bound $\mathbb{E}_{\Psi}[L]$
and $\sigma_{\Psi}[L]^2$ :
\begin{align}
\mathbb{E}_{\Psi}[L] \le& m \cdot (KL(p,q)+KL(q,p)) \cr 
&+ n \sum_{0\le i,j \le \frac{m}{2}-1}  {m/2-1 \choose i}{m/2-1 \choose
  j} \frac{p^{i+1}q^{j} + p^{j}q^{i+1}}{2} \log \frac{p^{i+1}q^{j} +
  p^{j}q^{i+1}}{p^{i}q^{j+1} + p^{j+1}q^{i}} \cr
\le& m \cdot (KL(p,q)+KL(q,p)) + n \sum_{1 \le k \le m}  m^k p^{k+1} k
\log \frac{p}{q} \cr
\le& O( \gamma f(n)) + np\log\frac{a}{b} \sum_{1 \le k \le m}  k m^k
p^{k} \le O( \gamma f(n)) + np\log\frac{a}{b} \sum_{k=1}^{\infty}  k
(mp)^{k}  \cr 
\le&O( \gamma f(n)) + np\log\frac{a}{b} \sum_{k=1}^{\infty}  
(2mp)^{k}   \cr
\sigma_{\Psi}[L]^2  \le &m( (p+q)(\log \frac{a}{b})^2 + (2-p-q)(\log\frac{1-q}{1-p})^2) \cr &+ n \sum_{0\le i,j \le \frac{m}{2}-1}  {m/2-1 \choose i}{m/2-1 \choose
  j} \frac{p^{i+1}q^{j} + p^{j}q^{i+1}}{2} \left(\log \frac{p^{i+1}q^{j} +
  p^{j}q^{i+1}}{p^{i}q^{j+1} + p^{j+1}q^{i}} \right)^2\cr
\le& 4m p (\log \frac{a}{b})^2 + n \sum_{1 \le k \le m}  m^k p^{k+1} k^2
(\log \frac{a}{b})^2 \cr 
\le& O(\gamma f(n)) + np (\log \frac{a}{b})^2 \sum_{k=1}^{\infty}
k^2 (mp)^{k} \le O(\gamma f(n)) + np (\log \frac{a}{b})^2 \sum_{k=1}^{\infty}
 (3mp)^{k} .
\end{align}
Therefore, the necessary condition for $\mathbb{E}_{\Psi}[L] +
2\sigma_{\Psi}[L] = \omega(1)$ is that $np \sum_{k=1}^{\infty}
 (3mp)^{k} = \omega(1)$. We conclude this proof from that $np \sum_{k=1}^{\infty}
 (3mp)^{k} = \omega(1)$ if and only if $\gamma f(n)^2 = \omega(1)$.

We now prove point (ii). Note that the probability for a red node to
be isolated is at least $(1-af(n)/n)^{\gamma n}\approx \exp(-a\gamma
f(n))$. If there exists an asymptotically accurate clustering
algorithm, then the fraction of such isolated red nodes should
vanishes and hence $\gamma f(n)\to \infty$.

\iffalse
\subsection{Proof of Theorem~\ref{th:3}}

We first consider case (i). We denote by $\Phi$ the true hidden partition $(V^{(g)}_k)_{1\le k
  \le K}$ for green nodes. Let
$\mathbb{P}_{\Phi}$ be the probability measure capturing the randomness
in the observations assuming that the network structure is described
by $\Phi$. We also introduce a slightly different structure
$\Psi$. The latter is described by clusters $V'^{(g)}_1 =V^{(g)}_1 \cup \{ v_2
\} \setminus \{ v_1
\}$, $V'^{(g)}_2=V^{(g)}_2 \cup \{v_1 \} \setminus \{ v_2 \}$, and $V'^{(g)}_k = V^{(g)}_k$ for all $3 \le k \le
K$ with arbitrary
selected $v_1\in V^{(g)}_1$ and $v_2 \in V^{(g)}_2$. With this
modification, let $V'_k = V'^{(g)}_k \cup V^{(r)}_k$. The observations intra- and
inter-cluster for nodes in $(V'_k)_{1\le k \le K} $ are generated as in
the initial SBM.

Let $\pi\in \Pi'$ denote a clustering algorithm for green nodes with
output $(\hat{V}^{(g)}_k)_{1\le k \le K}$, and let $\mathcal{E} =
\bigcup_{1\le k \le K}\hat{V}^{(g)}_k \setminus V^{(g)}_k$ be the set
of misclassified nodes under $\pi$. Note that in general in our
proofs, we always assume without loss of generality that $|
\bigcup_{1\le k \le K}\hat{V}^{(g)}_k \setminus V^{(g)}_k | \le |\bigcup_{1\le k
  \le K} \hat{V}^{(g)}_k \setminus V^{(g)}_{\gamma(k)}|$ for any permutation
$\gamma$, so that the set of misclassified nodes is really
$\mathcal{E}$. Further define $\mathcal{B}=\{ v_1 \in
\hat{V}^{(g)}_1\}$ as the set of events where node $v_1$ is
correctly classified under $\Phi$ and misclassified under $\Psi$. We have $\varepsilon (n) = |\mathcal{E}|$.

Let $x_{i,j}$ denote the label observed on node pair $(i,j)$. We
introduce $L$ (a quantity that resembles the log-likelihood ratio
between $\mathbb{P}_\Phi$ and $\mathbb{P}_{\Psi}$) as:
\begin{equation}L = \sum_{i \in V_1'}\log \frac{q(x_{i,v_1})p(x_{i,v_2})}{p(x_{i,v_1})q(x_{i,v_2})} + 
\sum_{i \in V_2'}\log \frac{p(x_{i,v_1})q(x_{i,v_2})}{q(x_{i,v_1})p(x_{i,v_2})},\end{equation}
In what follows, we establish a relationship between $\mathbb{E} [\varepsilon (n) ]$ and $L$. For any function $g(n)$, 
\begin{eqnarray} \label{eq:8-1}
\mathbb{P}_{\Psi} \{ L \le g(n) \}& =& \mathbb{P}_{\Psi} \{ L \le g(n) , \bar{\mathcal{B}} \} + \mathbb{P}_{\Psi} \{ L \le  g(n) , \mathcal{B} \}. 
\end{eqnarray}
We have: 
\begin{eqnarray}\mathbb{P}_{\Psi} \{ L \le  g(n) , \bar{\mathcal{B}}\} &= &
  \int_{\{ L \le g(n) , \bar{\mathcal{B}}\}} d\mathbb{P}_{\Psi} \cr
&= & \int_{\{ L \le g(n) , \bar{\mathcal{B}}\}} \prod_{i \in
  V_1'}\frac{q(x_{i, v_1})p(x_{i,v_2})}{p(x_{i,v_1})q(x_{i,v_2})}
\prod_{i \in V_2'}\frac{p(x_{i,v_1})q(x_{i,v_2})}{q(x_{i, v_1})p(x_{i,v_2})} d\mathbb{P}_{\Phi} \cr
&\le & \exp (g(n))\mathbb{P}_{\Phi} \{ L \le  g(n) , \bar{\mathcal{B}}\}~ \le ~ \exp (g(n))\mathbb{P}_{\Phi} \{ \bar{\mathcal{B}}\}\cr
&\le &\frac{1}{\alpha^{(g)}_1}\exp (g(n))\mathbb{E}_{\Phi} [ \varepsilon (n)],
\label{eq:bdl-1} \end{eqnarray}
where the last inequality comes from the fact that, since nodes in the
same community play identical roles,
$\mathbb{P}_{\Phi} \{ \mathcal{B} \} \ge 1- \mathbb{P}_{\Phi} \{ v_1 \notin
\hat{V}^{(g)}_1 \} \ge 1-\frac{1}{\alpha^{(g)}_1} \mathbb{E}_{\Phi}[ \varepsilon(n) ]. $
We also have: 
\begin{equation}\mathbb{P}_{\Psi} \{ L \le  g(n) , \mathcal{B} \} \le
  \mathbb{P}_{\Psi} \{  \mathcal{B} \} \le \frac{1}{\alpha^{(g)}_2}
  \mathbb{E}_{\Psi}[ \varepsilon(n) ] \le \frac{1}{4},
\label{eq:bdlf-1}
\end{equation} 
where the last ineqaulity stems from $\mathbb{E}_{\Psi}[
\varepsilon(n) ] = o(1)$.
Combining \eqref{eq:8-1},~\eqref{eq:bdl-1}, and \eqref{eq:bdlf-1}, we get
$$\mathbb{P}_{\Psi} \{ L \le  g(n) \} \le \frac{1}{\alpha^{(g)}_1}\mathbb{E}_{\Phi}[\varepsilon(n) ]\exp(g(n)) +
\frac{1}{4}. $$

Since  $\mathbb{E}_{\Phi}[\varepsilon(n) ] =\mathbb{E} [\varepsilon(n) ],$ choosing $g(n) = \log
\left( \frac{\alpha^{(g)}_1}{4 \mathbb{E} [ \varepsilon(n) ]} \right)$, we obtain:\begin{equation}\label{eq:infimum}
 \lim\inf_{n \rightarrow \infty}\mathbb{P}_{\Psi} \{ L \ge  \log \left( \frac{\alpha^{(g)}_1}{4 \mathbb{E} [ \varepsilon(n) ]} \right) \} \ge \frac{1}{2}. 
\end{equation}
By Chebyshev's inequality, $\mathbb{P}_{\Psi} \{ L \ge
\mathbb{E}_{\Psi}[L] + 2\sigma_{\Psi}[L] \} \le
\frac{1}{4}$. Therefore, to be valid the above inequality,
\begin{equation}
\mathbb{E}_{\Psi}[L] + 2\sigma_{\Psi}[L] \ge \log \left(\frac{\alpha^{(g)}_1}{4 \mathbb{E} [ \varepsilon(n,T) ]} \right).\label{eq:chevy}
\end{equation}
From the definition of $L$, we can easily bound $\mathbb{E}_{\Psi}[L]$
and $\sigma_{\Psi}[L]^2$ :
\begin{align}\label{eq:me2}
\mathbb{E}_{\Psi}[L] &\le (\alpha_1 + \alpha_2)n \cdot
(KL(q,p)+KL(q,p)) = O(f(n))\\ \label{eq:sig2}
\sigma_{\Psi}[L]^2 &\le q (\alpha_1 + \alpha_2)n \left(
    (p+q)(\log \frac{a}{b})^2 + (2-p-q)(\log\frac{1-q}{1-p})^2\right)
  = O(f(n)) .
\end{align}
The  statement of the theorem is then obtained by combining (\ref{eq:chevy}), (\ref{eq:me2}), and (\ref{eq:sig2}).


Now, we consider case (ii). When $\gamma = \Theta(1)$, 
$\frac{|\bigcup_{k} S^{(g)}_k \setminus V^{(g)}_k|}{|V^{(g)}|} = o(1)$
is necessary. Thus from case (i), $\gamma f(n)=\omega(1)$ is the
necessary condition. 

Consider that $\gamma = o(1)$. In this case, $\frac{|\bigcup_{k} S^{(r)}_k \setminus V^{(r)}_k|}{|V^{(r)}|} = o(1)$
is necessary, since $|V^{(r)}| = n(1-o(1))$. This proof is analogous
with the proof of case (i). Let $\Phi$ denote the
true partition for red nodes and $\Psi$ denote the slightly different
structure where $v_1 \in V^{(r)}_1$ and $v_2 \in V^{(r)}_2$ move to
$V^{(r)}_2$ and $V^{(r)}_1$, respectively. Then, $L$ is defined as
$$L = \sum_{i \in V^{(g)}_1}\log \frac{q(x_{v_1,i})p(x_{v_2,i})}{p(x_{v_1,i})q(x_{v_2,i})} + 
\sum_{i \in V^{(g)}_2}\log \frac{p(x_{v_1,i})q(x_{v_2,i})}{q(x_{v_1,i})p(x_{v_2,i})}.$$
As we did in (\ref{eq:chevy}) and (\ref{eq:me2}), we can bound
$\mathbb{E}_{\Psi}[L]$ and $\sigma_{\Psi}[L]^2$ as follows:
\begin{align*}
\mathbb{E}_{\Psi}[L] &\le (\alpha^{(g)}_1 + \alpha^{(g)}_2)m \cdot
(KL(q,p)+KL(q,p)) = O(\gamma f(n))\cr
\sigma_{\Psi}[L]^2 &\le q (\alpha^{(g)}_1 + \alpha^{(g)}_2)m \left(
    (p+q)(\log \frac{a}{b})^2 + (2-p-q)(\log\frac{1-q}{1-p})^2\right)
  = O(\gamma f(n)) .
\end{align*}
Therefore, $\gamma f(n) = \omega(1)$ is necessary to satisfy that
$\frac{|\bigcup_{1\le k \le K} S_k \setminus V_k |}{|V|} = o(1)$.
\fi

\subsection{Proof of Theorem~\ref{th:3}}

Let $M^{(g)} = \mathbb{E}[A^{(g)}] $ and $M' = \mathbb{E}[A'] .$ 
Let $A^{(g)}_{\Gamma} = (A^{(g)}_{vw})_{v,w\in \Gamma^{(g)}}$ and
$M^{(g)}_{\Gamma} = (M^{(g)}_{vw})_{v,w\in
  \Gamma^{(g)}}$. Analogously, we define $A'_{\Gamma}=
(A'_{vw})_{v,w\in \Gamma'}$ and $M'_{\Gamma}= (M'_{vw})_{v,w\in
  \Gamma'}$.  


\noindent{\bf \em Proof sketch)} The graph of indirect edges has the
same statistics as a SBM with these probabilities of connection since
the indirect edges are independent. Therefore, spectral methods will
work on both $A^{(g)}$ and $A'$ when the spectral norm of noise matrix
($A^{(g)}-M^{(g)}$ or $A'-M'$) is small compared to
the eigenvalues of $M^{(g)}$ and $M'$.  Roughly,
$\frac{\sigma_K^{(g)}}{\sqrt{m\hat{p}^{(g)}}}$ and
$\frac{\sigma'_K}{\sqrt{m\hat{p}'}}$ indicate signal over noise ratio
of $A^{(g)}$ and $A^{(g)}$, respectively.  As in \cite{yun2014}, we
can show that the
fraction of misclassified nodes is less than the inverse of the
signal over noise ratio (i.e., noise over signal) using spectral methods. This is why we
select one of the matrix $A^{(g)}$ or $A'$ according to the signal
over noise ratio in the algorithm. Therefore, showing that the signal
over noise ratio of the selected matrix grows up to infinity, we can
conclude the fraction of the misclassified nodes goes to
zero. Consider the case $\gamma f(n)=O(1)$.  In this case, it is easy
to see that the signal over noise ratio of the matrix $A'$ goes to
infinity as soon as $\sqrt{\gamma}f(n)=\omega(1)$, since the
probability of getting an indirect edge between two green nodes is of
the order $f(n)^2/n$.  Consider the case $\gamma f(n)=\omega(1)$. In
this case, the signal over noise ratio of the matrix $A^{(g)}$ goes to
infinity. Indeed, this proof consists of 2 steps: we show that in
\noindent{\em step 1)} 
$|\bigcup_{k=1}^K S^{(g)}_k \setminus V^{(g)}_k | = o ( |V^{(g)}| ) $
 using $A'$ when $\frac{\sigma'_K}{\sqrt{m \hat{p}'}} \cdot 1_{\{
  m \hat{p}' \ge 50\}} = \omega(1)$ and  using $A^{(g)}$ when
$\frac{\sigma^{(g)}_K}{\sqrt{m \hat{p}^{(g)}}} \cdot 1_{\{ m
  \hat{p}^{(g)} \ge 50\}} = \omega(1)$ and in 
\noindent{\em step 2)} 
$\max\{ \frac{\sigma^{(g)}_K}{\sqrt{m \hat{p}^{(g)}}} \cdot 1_{\{ m
    \hat{p}^{(g)} \ge 50\}},
  \frac{\sigma'_K}{\sqrt{m \hat{p}'}} \cdot 1_{\{ m \hat{p}' \ge
    50\}} \} =\omega(1).$
Then, from the results of step 1 and step 2, we conclude that the
output of Algorithm~1 classifies green nodes accurately.
In what follows, we will give exact proofs for each step.

\vspace{0.5cm}
\noindent{\bf \em Step 1)} Since the proofs are
analogous, we provide only the proof of  the first case, which assumes
that $\frac{\sigma'_K}{\sqrt{m \hat{p}'}} \cdot 1_{\{
  m \hat{p}' \ge 50\}} = \omega(1)$. In this step, we
denote by $M'_{\Gamma} = U \Lambda U^T$ the factorization form of the
singular value decomposition of $M'_{\Gamma}$ and $U_\bot$ 
an orthonormal basis of the perpendicular space to the linear span of
$U$.  

First, we will show that $\frac{\sigma'_K}{\sqrt{m \hat{p}'}} \cdot 1_{\{
  m \hat{p}' \ge 50\}} = \omega(1)$ implies that exact signal over noise ratio $\frac{\lambda_K
  (M_{\Gamma}')}{\|A'_{\Gamma} - M'_{\gamma} \|} = \omega(1)$ from
$\|A'_{\Gamma} - M'_{\gamma} \| = O(\sqrt{m \hat{p}'})$ and $\lambda_K
  (M_{\Gamma}') = \Theta( \sigma'_K )$.  With high probability, $\hat{p}' = \frac{\sum_{uv}
  M'_{uv}}{m^2} = \Theta( \max_{uv} \{ M_{uv} \})$ by the law of large
number and $\sum_{w \in \Gamma'} A'_{vw} =O(m\hat{p}')$ for all $v\in \Gamma'$ by the trimming process in Approx algorithm.
Thus, from the random matrix theory \cite{feige2005spectral}, with probability $1-O(1/m)$, $\|A'_{\Gamma} - M'_{\Gamma} \| =
O(\sqrt{m \hat{p}'})$. Since we show that $\sigma'_K =
\Theta(\lambda_K(A'_{\Gamma}))$ in Lemma~\ref{lem:powersing} and $\lambda_K(M'_{\Gamma}) \ge
\lambda_K(A'_{\Gamma}) -\|A'_{\Gamma} - M'_{\Gamma} \|$,
$\frac{\sigma'_K}{\sqrt{m \hat{p}'}}  = \omega(1)$. 
\begin{lemma}
With probability $1-O(1/|V|)$, the output $(Q,\sigma_K)$ of Power Method
$(A,V,K)$ (Algorithm~\ref{alg:pm}) satisfies that $\sigma_K = \Theta (\lambda_K (A))$.\label{lem:powersing}
\end{lemma}
Therefore, we deduce that 
$$\frac{\lambda_K
  (M'_\Gamma)}{\|A'_{\Gamma} -M'_{\Gamma} \|}
= \omega(1) .$$ 

Lemma~\ref{lem:poweriter} implies that when $A'_\Gamma$ is close to $M'_{\Gamma}$, the
linear span of $Q'$, the eigenvectors of $A'_\Gamma$ corresponding to the
$K$ largest eigenvalues, is also close to the linear span of
$U$.
\begin{lemma} Let $A$ and $M$ be $V \times V$ matrices and $M=U
  \Lambda U^T$ be the SVD of $M$ where $\Lambda \in
  \mathbb{R}^{K\times K}$.  When $\|A-M \|= o \left( \lambda_K ( M )
  \right)$, the output $(\sigma_K, Q)$ of the power method (Algorithm~\ref{alg:pm}) with input $(A,V,K)$ satisfies that
$\| U_{\bot}^T Q \| =O\left( \frac{\|A-M \| }{\lambda_K (M)}
\right) = o(1) $, where $U_{\bot}$ is an orthonormal basis of the
perpendicular space to the linear span of $U$. \label{lem:poweriter}
\end{lemma}
 Since $\frac{\lambda_K (M'_{\Gamma} )}{
  \|A'_{\Gamma} - M'_{\Gamma} \| } = \omega(1)$ with probability
$1-O(1/m)$, by Lemma~\ref{lem:poweriter}, the output $Q'$ of Power Method
with input $(A'_{\Gamma},V, K)$ (Algorithm~\ref{alg:pm}) satisfies
that 
\begin{equation}\|
  U_{\bot}^T Q' \| = o(1) \quad \mbox{w.p.}\quad 1-O(1/m) .\label{eq:uqd} \end{equation}

We will conclude this step by showing that $| V^{(g)} \setminus
\Gamma' | = o ( |V^{(g)}| )$ and $|(\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k ) \bigcap \Gamma'| =  o ( |V^{(g)}| )$. It is easy
to check $| V^{(g)} \setminus \Gamma' | = o ( |V^{(g)}| )$ by showing
$m\hat{p}' = \omega(1)$, since $| V^{(g)} \setminus
\Gamma' | = m\exp(-m\hat{p}')$ in Algorithm~\ref{alg:trim}. Since $\frac{\lambda_K
  (A'_\Gamma)}{\|A'_{\Gamma} -M'_{\Gamma} \|}
= \omega(1) $ and $\|A'_{\Gamma} -M'_{\Gamma} \| = \Omega(1)$, $\| A'_\Gamma
\| = \omega(1)$ and thus $m\hat{p}' = \omega(1)$. For the remaining
part $|(\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k ) \bigcap \Gamma'| =  o ( |V^{(g)}| )$, we
introduces Lemma~\ref{lem:detection}, where we show that the fraction
of misclassified nodes is less than $\|  U_{\bot}^T Q' \|$.
\begin{lemma}For given set $V$ with partition $(V_k)_{1\le k \le K}$
  such that $\frac{|V_k|}{|V|}$ is constant for all $k$, let $U_B $ be the $V \times K$ matrix where $(v,k)$ element is
$1/\sqrt{|V_k|}$ when $v\in V_k$ for all $k$ and $0$ otherwise. Let
$U_{\bot}$ be an orthonormal basis of the perpendicular space to the
linear span of $U_B$. The output $(S_k)_{1\le k \le K}$ of Detection$(Q,V,K)$
  satisfies that when $\|U_{\bot}^T Q \| = o(1)$
 $$\frac{\left| \bigcup_{k=1}^K S_k
\setminus V_k \right|}{|V|} = O \left( \|U_{\bot}^T Q \|^2\right).$$\label{lem:detection}
\end{lemma}
As in Lemma~\ref{lem:detection}, we denote by $U_B $ the $\Gamma' \times K$ matrix where $(v,k)$ element is
$1/\sqrt{|V_k \bigcap \Gamma'|}$ when $v\in (V_k \bigcap \Gamma' )$
for all $k$ and $0$ otherwise. Since the rows of $M_{\Gamma}' x$
are distinct according to the clusters for any $x \in
\mathbb{R}^{\Gamma' \times 1}$,  the linear span of $U$ coincides with the linear span of
$U_B$. In addition, we know that $\|U_\bot^{T} Q'\| = o(1)$ from \eqref{eq:uqd}. From Lemma~\ref{lem:detection}, therefore, $|(\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k ) \bigcap \Gamma'| = o ( |\Gamma'| ) = o (
|V^{(g)}| )$. This is the end of the proof of this step.


\vspace{0.5cm}
\noindent{\bf \em Step 2)} In this step, we consider two cases $\gamma f(n) =
\omega(1)$ and $\gamma f(n) =
O(1)$. We conclude this step from that $\frac{\sigma^{(g)}_K}{\sqrt{m \hat{p}^{(g)}}} \cdot 1_{\{ m
    \hat{p}^{(g)} \ge 50\}} = \omega(1)$ when $\gamma f(n) =
\omega(1)$ and $\frac{\sigma'_K}{\sqrt{m \hat{p}'}} \cdot 1_{\{ m
    \hat{p}' \ge 50\}} = \omega(1)$ when $\gamma f(n) =
O(1)$ and $\sqrt{\gamma }f(n) =
\omega(1)$.

Consider $\gamma f(n) =
\omega(1)$. With high probability, by the law of
large numbers, $m\hat{p}^{(g)} = \Theta(\gamma f(n))$.
Since $\lambda_K (M_{\Gamma}^{(g)}) = \Omega(\gamma f(n))$, 
$\| A^{(g)}_{\Gamma} - M^{(g)}_{\Gamma}\| =
\Theta(\sqrt{m\hat{p}^{(g)}}) = \Theta(\sqrt{\gamma f(n)})$ and $\lambda_{K}(A_{\Gamma}^{(g)}) \ge
\lambda_{K}(M_{\Gamma}^{(g)}) -\|A_{\Gamma}^{(g)}-M_{\Gamma}^{(g)} \|$, $\frac{\lambda_K
  (A_{\Gamma}^{(g)})}{\sqrt{ m \hat{p}^{(g)}
  }} = \omega(1)$. Since $\sigma^{(g)}_{K} =
\Theta (\lambda_K  (A_{\Gamma}^{(g)}))$ from Lemma~\ref{lem:powersing}, 
$$\frac{\sigma^{(g)}_{K}}{\sqrt{m\hat{p}^{(g)}}}\cdot 1_{\{ m
    \hat{p}^{(g)} \ge 50\}} = \omega(1). $$


Consider $\gamma f(n)= O(1)$ and $\gamma f(n)^2= \omega(1)$. We first compute the elements of $M'_{ij}$.  For notational simplicity, let $\alpha_k$ and $\beta_k$
denote $\frac{|V^{(g)}_{k}|}{n}$ and $\frac{|V^{(r)}_{k}|}{n}$. Let
nodes $i$ and $j$ be in $V^{(g)}_k$. For $v\in V^{(r)}_k ,$ the
probability of that $\sum_{w \in V^{(g)}} a_{vw} = 2$ (i.e., the red
node has two connections with green nodes) and the two green nodes are
$i$ and $j$ is $p^2 (1-p)^{\beta_k n -2} \prod_{k' \neq k}
(1-q)^{\beta_{k'}n}$. As $n\to \infty$, the probability converges to
$p^2 \exp(-\alpha_k p n- \sum_{i\neq k} \alpha_i qn).$ For $v \in
V^{(r)}_{k'}$, the probability of that $\sum_{w \in V^{(g)}} a_{vw} =
2$ and the two green nodes are $i$ and $j$ is $q^2 \exp(-\alpha_{k'} p
n- \sum_{i\neq k'} \alpha_i qn)$ analogously. Let $\eta_k =
\exp(-\alpha_k p n- \sum_{i\neq k} \alpha_i qn)$. Since $|V^{(r)}_k|
=\beta_n n,$ when $i$ and $j$ are in $V^{(g)}_k ,$
\begin{equation}
m'_{ij} =
p^2 \beta_k \eta_k n  + q^2 n \sum_{k' \neq k} \beta_{k'}
\eta_{k'}. \label{eq:mkk}
\end{equation}
Let $i \in V_k$ and $j\in V_\ell$. For $v \in V^{(r)}_k \cup
V^{(r)}_\ell$, since both $i$ and $j$ have connections with $v$ with
probability $pq$ and for  $v \notin V^{(r)}_k \cup
V^{(r)}_\ell$ the probability is $q^2$,
\begin{equation}
m'_{ij} = pq (\beta_k \eta_k  + \beta_\ell \eta_\ell )n  + q^2 n \sum_{k'
  \notin \{k,\ell\}} \beta_{k'} \eta_{k'}. \label{eq:mij}
\end{equation}
Thus, we can represent $M'$ as follows:
$$ M'_\Gamma = M^{(g)}_{\Gamma' , K}\cdot \Lambda' \cdot
(M^{(g)}_{\Gamma' , K})^T ,$$
where $M^{(g)}_{\Gamma' , K}$ is a $\Gamma' \times K$ matrix where
the $k$-th column of $M^{(g)}_{\Gamma' , K}$ is the column vector of
$M^{(g)}_{\Gamma}$ corresponding to $ v \in V^{(g)}_k$, and $\Lambda'$ is a $K\times K$ diagonal
matrix where $k$-th element is $\beta_k
\eta_k n$. Since $\frac{\|M^{(g)}_{\Gamma' , K} {\boldsymbol x}
  \|}{\|{\boldsymbol x}\|} = \Omega(\sqrt{m}p)$ for any ${\boldsymbol x}\in \mathbb{R}^{K\times 1}$, $\lambda_K (M'_{\Gamma}) = \Omega (mnp^2 \min\limits_{1\le k \le
  K} \eta_k ) = \Omega(\gamma f(n)^2)$. By law of large number, with
high probability, $m\hat{p}' = \Theta( \frac{\gamma}{n}f(n)^2
)$. Then, analogously with the previous case ($\gamma f(n) =
\omega(1)$), we conclude that 
$$\frac{\sigma'_{K}}{\sqrt{m\hat{p}'}}\cdot 1_{\{ m
    \hat{p}' \ge 50\}} = \omega(1). $$

\iffalse
\noindent{\em step 1)} In this step, we will show that the adjacency
matrix $A'_\Gamma$ induced by the indirect edges does
not deviate much from $M'_{\Gamma}$ compared to the singular values of
$M'_{\Gamma}$. Indeed, from random matrix theory (Feige and Ofek), we
show that with probability $1-O(1/m)$, $\frac{\lambda_K
  (M'_\Gamma)}{\|A'_{\Gamma} -M'_{\Gamma} \|}
= \omega(1)$. Recall that $\lambda_K (M'_\Gamma)$ is the $K$-th largest
singular value. 

\noindent{\em step 2)} When $A'_\Gamma$ is close to $M'_{\Gamma}$, the
linear span of $Q$, the eigenvectors of $A'_\Gamma$ corresponding to the
$K$ largest eigenvalues, is also close to the linear span of
$U$. In this step, we show that $\|U_{\bot}^{T} Q' \| = o(1)$ when $\frac{\lambda_K
  (M'_\Gamma)}{\|A'_{\Gamma} -M'_{\Gamma} \|}
= \omega(1)$.

\noindent{\em step 3)} This step concludes this theorem. Since the
rows of $U$ corresponding to the same cluster are the same and the
linear span $Q$ is almost the same with the linear span of $U$, we can
find clusters from the rows of $Q$.  In this step, we show that
$|\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k | = o ( |V^{(g)}| ) $ when $\|U_{\bot}^{T} Q' \| = o(1)$. 




\vspace{0.5cm}
\noindent{\bf \em Step 1)} The goal of this step is showing
$\frac{\lambda_{K}(M'_{\Gamma})}{ \|A'_{\Gamma} - M'_{\Gamma}
  \|}=\omega(1)$. With high probability, $\hat{p}' = \frac{\sum_{uv}
  M'_{uv}}{m^2} = \Theta( \max_{uv} \{ M_{uv} \})$ by law of large
number.  Since $|V^{(g)}\setminus \Gamma'| = |V^{(g)}| \exp (- c
|V^{(g)}| \max_{uv} \{ M_{uv} \})$ with some constant $c$, one can
easily show that $x_{v} = O(m\hat{p}')$ for all $v\in \Gamma'$ by
Chernoff bound. Therefore, by the random matrix theory (Feige and
Ofek), with probability $1-O(1/m)$, $\|A'_{\Gamma} - M'_{\Gamma} \| =
O(\sqrt{m \hat{p}'})$. Analogously, when $m\hat{p}^{(g)} \ge 50$, with
probability $1-O(1/m)$, $\|A_{\Gamma}^{(g)}-M_{\Gamma}^{(g)} \| =
O(\sqrt{mp}) = O(\sqrt{\gamma f(n)})$.


First, consider $\gamma f(n) = \omega(1)$. In this case,
$\frac{\sigma^{(g)}_{K}}{\sqrt{m\hat{p}^{(g)}}} = \omega(1)$ with the
following reasons. Since $\lambda_K (M_{\Gamma}^{(g)}) =
\Omega(\gamma f(n))$ and $\sqrt{m\hat{p}^{(g)}} =
\Theta(\sqrt{\gamma f(n)})$ by the law of large numbers, $\frac{\lambda_K
  (M_{\Gamma}^{(g)})}{\sqrt{m\hat{p}^{(g)}}} = \omega(1)$. Since
$\lambda_{K}(A_{\Gamma}^{(g)}) \ge \lambda_{K}(M_{\Gamma}^{(g)}) 
-\|A_{\Gamma}^{(g)}-M_{\Gamma}^{(g)} \|$  and $\lambda_{K+1}
(A_{\Gamma}^{(g)}) \le \|A_{\Gamma}^{(g)}-M_{\Gamma}^{(g)} \|$, from Lemma~\ref{lem:powersing}, $\sigma^{(g)}_{K} =
\Omega(\gamma f(n)) $ and thus 
$\frac{\sigma^{(g)}_{K}}{\sqrt{m\hat{p}^{(g)}}} = \omega(1)$. 
Since we consider $\frac{\sigma^{(g)}_K}{\sqrt{m \hat{p}^{(g)}}}
\le \frac{\sigma'_K}{\sqrt{m \hat{p}'}}$, $\frac{\sigma'_K}{\sqrt{m
    \hat{p}'}}= \omega(1)$. We conclude $\frac{\lambda_{K}(M'_{\Gamma})}{ \|A'_{\Gamma} -
  M'_{\Gamma} \|}=\omega(1)$, from $\|A'_{\Gamma} - M'_{\Gamma} \|=
O(\sqrt{m \hat{p}'})$ and Lemma~\ref{lem:powersing}.

% \begin{lemma} For any set $\tilde{V}$ with partition
%   $(\tilde{V}_k)_{1\le k\le K}$ such that $\frac{|V|}{|V_k|}$ is a finite constant for all cluster $k$, let $\tilde{M}$ be a $\tilde{V}
%   \times \tilde{V}$ matrix where $\tilde{M}_{vw} = p$ when $v$ and $w$ are from the same cluster and
% $\tilde{M}_{vw}=q$ when $v$ and $w$ are from different clusters. 
% $\lambda_K (\tilde{M}) = \Omega(p|\tilde{V}|)$.\label{lem:Ksingular}
% \end{lemma}
\begin{lemma}
With probability $1-O(1/|V|)$, the output $(Q,\sigma_K)$ of Power Method
$(A,V,K)$ (Algorithm~\ref{alg:pm}) satisfies that $\sigma_K = \Theta (\lambda_K (A))$.\label{lem:powersing}
\end{lemma}




Consider $\gamma f(n)= O(1)$. We first compute the elements of $M'_{ij}$.  For notational simplicity, let $\alpha_k$ and $\beta_k$
denote $\frac{|V^{(g)}_{k}|}{n}$ and $\frac{|V^{(r)}_{k}|}{n}$. Let
nodes $i$ and $j$ be in $V^{(g)}_k$. For $v\in V^{(r)}_k ,$ the
probability of that $\sum_{w \in V^{(g)}} a_{vw} = 2$ (i.e., the red
node has two connections with green nodes) and the two green nodes are
$i$ and $j$ is $p^2 (1-p)^{\beta_k n -2} \prod_{k' \neq k}
(1-q)^{\beta_{k'}n}$. As $n\to \infty$, the probability converges to
$p^2 \exp(-\alpha_k p n- \sum_{i\neq k} \alpha_i qn).$ For $v \in
V^{(r)}_{k'}$, the probability of that $\sum_{w \in V^{(g)}} a_{vw} =
2$ and the two green nodes are $i$ and $j$ is $q^2 \exp(-\alpha_{k'} p
n- \sum_{i\neq k'} \alpha_i qn)$ analogously. Let $\eta_k =
\exp(-\alpha_k p n- \sum_{i\neq k} \alpha_i qn)$. Since $|V^{(r)}_k|
=\beta_n n,$ when $i$ and $j$ are in $V^{(g)}_k ,$
\begin{equation}
m'_{ij} =
p^2 \beta_k \eta_k n  + q^2 n \sum_{k' \neq k} \beta_{k'}
\eta_{k'}. \label{eq:mkk}
\end{equation}
Let $i \in V_k$ and $j\in V_\ell$. For $v \in V^{(r)}_k \cup
V^{(r)}_\ell$, since both $i$ and $j$ have connections with $v$ with
probability $pq$ and for  $v \notin V^{(r)}_k \cup
V^{(r)}_\ell$ the probability is $q^2$,
\begin{equation}
m'_{ij} = pq (\beta_k \eta_k  + \beta_\ell \eta_\ell )n  + q^2 n \sum_{k'
  \notin \{k,\ell\}} \beta_{k'} \eta_{k'}. \label{eq:mij}
\end{equation}
Thus, we can represent $M'$ as follows:
$$ M'_\Gamma = M^{(g)}_{\Gamma' , K}\cdot \Lambda' \cdot
(M^{(g)}_{\Gamma' , K})^T ,$$
where $M^{(g)}_{\Gamma' , K}$ is a $\Gamma' \times K$ matrix where
the $k$-th column of $M^{(g)}_{\Gamma' , K}$ is the column vector of
$M^{(g)}_{\Gamma}$ corresponding to $ v \in V^{(g)}_k$, and $\Lambda'$ is a $K\times K$ diagonal
matrix where $k$-th element is $\beta_k
\eta_k n$. Since $\frac{\|M^{(g)}_{\Gamma' , K} {\boldsymbol x}
  \|}{\|{\boldsymbol x}\|} = \Omega(\sqrt{m}p)$ for any ${\boldsymbol x}\in \mathbb{R}^{K\times 1}$, $\lambda_K (M'_{\Gamma}) = \Omega (mnp^2 \min\limits_{1\le k \le
  K} \eta_k ) = \Omega(\gamma f(n)^2)$  and thus
$\frac{\lambda_K (M'_{\Gamma})}{ \| A'_{\Gamma} - M'_{\Gamma} \| } = \Omega
(\sqrt{\gamma}f(n))= \omega(1)$.

\vspace{0.5cm}
\noindent{\bf \em Step 2)} We conclude this step with
Lemma~\ref{lem:poweriter}.  Since $\frac{\lambda_K (M'_{\Gamma} )}{
  \|A'_{\Gamma} - M'_{\Gamma} \| } = \omega(1)$ with probability
$1-O(1/m)$ from the previous step, the output $Q'$ of Power Method
with input $(A'_{\Gamma},V, K)$ (Algorithm~\ref{alg:pm}) satisfies that $\|
U_{\bot}^T Q' \| = o(1)$ with probability $1-O(1/m)$ by Lemma~\ref{lem:poweriter}.
\begin{lemma} Let $A$ and $M$ be $V \times V$ matrices and $M=U
  \Lambda U^T$ be the SVD of $M$ where $\Lambda \in
  \mathbb{R}^{K\times K}$.  When $\|A-M \|= o \left( \lambda_K ( M )
  \right)$, the output $(\sigma_K, Q)$ of the power method (Algorithm~\ref{alg:pm}) with input $(A,V,K)$ satisfies that
$\| U_{\bot}^T Q \| =O\left( \frac{\|A-M \| }{\lambda_K (M)}
\right) = o(1) $, where $U_{\bot}$ is an orthonormal basis of the
perpendicular space to the linear span of $U$. \label{lem:poweriter}
\end{lemma}

% \begin{lemma}Let $M = U\Lambda U^T$ be the SVD of $M$ where $\Lambda
%   \in \mathbb{R}^{K \times K}$ and $Q \Lambda^{\star} Q^T$ be the SVD of the
%   $K$ rank approximation of $(M+X)$. Then, $\|U_{\bot}^{T} Q \| \le
%   \frac{\|X \|}{\lambda_K (M)-\|X \|}$. \label{lem:QU}
% \end{lemma}
% The
%  proof of Lemma~\ref{lem:QU} is provided in Section~\ref{sec:proof-lemma-refl}.


\vspace{0.5cm}
\noindent{\bf \em Step 3)} In this step, we will show that $| V^{(g)} \setminus
\Gamma' | = o ( |V^{(g)}| )$ and $|(\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k ) \bigcap \Gamma'| =  o ( |V^{(g)}| )$ to conclude
$|\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k | = o ( |V^{(g)}| ) $. First, since we remove $m\exp(-m\hat{p}')$
nodes in Algorithm~\ref{alg:trim} and $m\hat{p}' = \omega(1)$, $| V^{(g)} \setminus
\Gamma' | = o ( |V^{(g)}| )$. We exploits Lemma~\ref{lem:detection} to
show the second term. As in the lemma, we denote by $U_B $ the $\Gamma' \times K$ matrix where $(v,k)$ element is
$1/\sqrt{|V_k \bigcap \Gamma'|}$ when $v\in (V_k \bigcap \Gamma' )$
for all $k$ and $0$ otherwise. Since the rows of $M_{\Gamma}' x$
corresponding to the same cluster are the same for any $x \in
\mathbb{R}^{\Gamma' \times 1}$,  the linear span of $U$ coincides with the linear span of
$U_B$. In addition, we know that $\|U_\bot^{T} Q'\| = o(1)$ from the
previous step. From Lemma~\ref{lem:detection}, therfore, $|(\bigcup_{k=1}^K S^{(g)}_k
\setminus V^{(g)}_k ) \bigcap \Gamma'| = o ( |\Gamma'| ) = o (
|V^{(g)}| )$. This is the end of this proof.

\begin{lemma}For given set $V$ with partition $(V_k)_{1\le k \le K}$
  such that $\frac{|V_k|}{|V|}$ is constant for all $k$, let $U_B $ be the $V \times K$ matrix where $(v,k)$ element is
$1/\sqrt{|V_k|}$ when $v\in V_k$ for all $k$ and $0$ otherwise. Let
$U_{\bot}$ be an orthonormal basis of the perpendicular space to the
linear span of $U_B$. The output $(S_k)_{1\le k \le K}$ of Detection$(Q,V,K)$
  satisfies that when $\|U_{\bot}^T Q \| = o(1)$
 $$\frac{\left| \bigcup_{k=1}^K S_k
\setminus V_k \right|}{|V|} = O \left( \|U_{\bot}^T Q \|^2\right).$$\label{lem:detection}
\end{lemma}

\fi

\subsection{Proof of Theorem~\ref{thm:clust-algor-red}}
By Theorem~\ref{th:3}, $|\bigcup_{k=1}^K (S^{(g)}_k
\setminus V^{(g)}_k ) | =o(|V^{(g)}|) .$ Let $\mu ( v, S^{(g)}_k ) =
\mathbb{E} [ \sum_{w \in S^{(g)}_k} A_{vw}]$. Then,  $\frac{\mu ( v,
  S^{(g)}_k )}{|S^{(g)}_k|} = p(1+ o(1))$ when $v\in V_k$ and $\frac{\mu ( v,
  S^{(g)}_k )}{|S^{(g)}_k|} = q(1+ o(1))$ when $v\notin V_k$. By the
Chernoff bound, therefore, $v \in S_k$ when $v \in V_k$ with
probability $1-\exp(-c_1 p |V^{(g)}|)$ with positive constant $c_1>0$.

\subsection{Proof of Theorem~\ref{thm:streaming-with-green}}
From Theorem~\ref{th:3}, 
Algorithm~1 classifies the arrival nodes at each time
block with diminishing fraction of misclassified nodes. Between
$S^{(\tau)}_i$ and $S^{(\tau+1)}_j$, the number of connections is
$\Theta( B^2 \frac{\bar{f}(n)}{n}) = \Theta( \frac{h^2(n)n}{\min\{f(n),n^{1/3} \} \log^2 n}) = \omega(1)$ from
the condition of this theorem. Let $\mu(k,i) = \frac{ \sum_{v \in \hat{V}_i}\sum_{w \in
  S^{(\tau)}_{k}} A_{wv}}{ \sum_{v \in \hat{V}_i}\sum_{w \in
  S^{(\tau)}_{k}} 1}$. By the Chernoff bound,
with high probability (since $\sum_{v \in \hat{V}_i}\sum_{w \in
  S^{(\tau)}_{k}} A_{wv} =\omega(1)$),  $\mu(k,i) =p(1-o(1))$ when $\frac{|S^{(\tau)}_k
  \bigcap V_i|}{|S^{(\tau)}_k|} = 1-o(1)$ and $\mu(k,i) =q(1+o(1))$ when $\frac{|S^{(\tau)}_k
  \bigcap V_i|}{|S^{(\tau)}_k|} = o(1)$. Therefore, with high
probability, $S^{(\tau)}_k$ is merged with $\hat{V}_{s(k)}$ such that $\frac{|S^{(\tau)}_k \bigcap V_{s(k)}|}{|S^{(\tau)}_k|} =
1-o(1)$. Thus, $\frac{|\hat{V}_k \bigcap V_{k}|}{|\hat{V}_k|} =
1-o(1)$ for all $k$ with high probability. 

Now, consider that $\frac{|\hat{V}_k \bigcap V_{k}|}{|\hat{V}_k|} =
1-o(1)$ for all $k$.  Since $\frac{|\hat{V}_k \bigcap V_{k}|}{|\hat{V}_k|} =
1-o(1)$ for all $k$, one can easily show using Chernoff bound that $\frac{N_{v,k}}{|\hat{V}_k|} \ge p(1-\frac{p-q}{4})$ when $v
\in V_k$ and $\frac{N_{v,k}}{|\hat{V}_k|} \le q(1+\frac{p-q}{4})$ when $v
\notin V_k$ with probability $1-O(\exp (-c p T) )$ with positive constant
$c>0$. Thus, when $T =\omega(\frac{n}{f(n)}) $, the error
probability is $O(\exp(-T\frac{f(n)}{n}))$.



\subsection{Proof of Lemma~\ref{lem:powersing}}

{\em i) $\sigma_K = O(\lambda_K(A))$ : } When $\|A\| = \Theta (\lambda_K(A))$, this is trivial since
singular values of $R_{\tau^{\star}}$ have to be less than $\|A\|$.
Let $\lambda_{i}(A) = \omega(\lambda_K(A))$ and $\lambda_{i+1}(A) =
\Theta(\lambda_K(A))$. We denote by $\tilde{U}_j \tilde{\Lambda} \tilde{U}_j^T$ be the SVD of rank $j$
approximation of $A$.  Let $Q_{j,\tau^{\star}}$ denote the $j$-th column
vector of $Q_{\tau^{\star}}$. Analogously with part {\em i)} of the
proof of Lemma~\ref{lem:poweriter} (Please refer to part {\em i)}  of
the proof for the details), we can show that
$\|\tilde{U}_{j}^T Q_{K,\tau^{\star}}\| = O(\frac{\lambda_K
  (A)}{\lambda_{j}(A)})$ for all $j \le i$. Therefore, $\sigma_{k} = O(\lambda_K(A))$.

{\em ii) $\sigma_K = \Omega(\lambda_K(A))$ : } When $\lambda_{|V|}(A) = \Theta (\lambda_K(A))$, this is trivial since
singular values of $R_{\tau^{\star}}$ have to be larger than $\lambda_{|V|}(A)$.
Let $\lambda_{i+1}(A) = o(\lambda_K(A))$ and $\lambda_{i}(A) =
\Theta(\lambda_K(A))$. Analogously with part {\em i)} of the
proof of Lemma~\ref{lem:poweriter}, we can show that
$\|(\tilde{U}_{i})_{\bot}^T Q_{K,\tau^{\star}}\| = O(\frac{\lambda_i
  (A)}{\lambda_{i+1}(A)})$, where $(\tilde{U}_{i})_{\bot}$ is an
orthonormal basis of the perpendicular to the linear span of
$\tilde{U}_{i}$. Therefore, $\sigma_{k} = \Omega (\lambda_i (A)) =
\Omega (\lambda_K (A))$.



\subsection{Proof of Lemma~\ref{lem:poweriter}}
We denote by $\tilde{U} \tilde{\Lambda} \tilde{U}^T$ be the SVD of rank $K$
approximation of $A$. Let $U_\bot$ and $\tilde{U}_\bot$ be orthonormal bases of
the perpendicular spaces to the linear spans of $U$ and $\tilde{U}$, respectively. 
Since
\begin{align*}
\|U_{\bot}^T Q_{\tau^{\star}} \| & = \|U_{\bot}^T (\tilde{U}\tilde{U}^T +
\tilde{U}_{\bot}\tilde{U}_{\bot}^T )Q_{\tau^{\star}} \| \le \|U_{\bot}^T
\tilde{U}\tilde{U}^T Q_{\tau^{\star}} \| + \|U_{\bot}^T
\tilde{U}_{\bot}\tilde{U}_{\bot}^T Q_{\tau^{\star}} \| \cr
& \le \|U_{\bot}^T\tilde{U}\| \|\tilde{U}^T Q_{\tau^{\star}} \| + \|U_{\bot}^T
\tilde{U}_{\bot} \| \| \tilde{U}_{\bot}^T Q_{\tau^{\star}} \| \le \|U_{\bot}^T\tilde{U}\| +  \| \tilde{U}_{\bot}^T Q_{\tau^{\star}} \|,
\end{align*}
to conclude this proof, we will show that $\| \tilde{U}_{\bot}^T
Q_{\tau^{\star}} \| =O\left( \frac{\|A-M \| }{\lambda_K (M)} \right)$ and $\|U_{\bot}^T\tilde{U}\| = O\left( \frac{\|A-M \| }{\lambda_K (M)}
\right)$.

\noindent\underline{\em i) $\| \tilde{U}_{\bot}^T
Q_{\tau^{\star}} \| =O\left( \frac{\|A-M \| }{\lambda_K (M)} \right)$:}Let $\boldsymbol{x}_1$ be the right singular vector of $\tilde{U}_{\bot}^T Q_{\tau + 1}$
corresponding to the largest singular value. Then,
\begin{align}
\|\tilde{U}_{\bot}^T Q_{\tau + 1} \|_2^2 &= \frac{\|\tilde{U}_{\bot}^T Q_{\tau + 1}
  \boldsymbol{x}_1 \|_2^2}{\|\boldsymbol{x}_1\|^2_2} =
\frac{\|\tilde{U}_{\bot}^T Q_{\tau + 1} R_{\tau+1}
  \tilde{\boldsymbol{x}}_1 \|_2^2}{\|R_{\tau+1}\tilde{\boldsymbol{x}}_1\|^2_2} \cr&=\frac{\|\tilde{U}_{\bot}^T Q_{\tau + 1} R_{\tau+1}
  \tilde{\boldsymbol{x}}_1
  \|_2^2}{\|\tilde{U}^T Q_{\tau+1} R_{\tau+1}\tilde{\boldsymbol{x}}_1\|^2_2 + \|\tilde{U}_{\bot}^T Q_{\tau+1} R_{\tau+1}\tilde{\boldsymbol{x}}_1\|^2_2} \cr&=\frac{\|\tilde{U}_{\bot}^T AQ_{\tau }
  \tilde{\boldsymbol{x}}_1
  \|_2^2}{\|\tilde{U}^T AQ_{\tau }\tilde{\boldsymbol{x}}_1\|^2_2 +
  \|\tilde{U}_{\bot}^T AQ_{\tau }\tilde{\boldsymbol{x}}_1\|^2_2} \cr
&\le  \frac{\|A -M \|_2^2}{ (\lambda_K (M) - \|A -M \|_2 )^2 (1- \|\tilde{U}_{\bot}^T
  Q_{\tau} \|_2^2) +   \|A -M \|_2^2} , \label{eq:uqbnd}
\end{align}
where the last inequality stems from that
\begin{align*}
\|\tilde{U}_{\bot}^T AQ_{\tau }  \tilde{\boldsymbol{x}}_1  \|_2  
&\le \| \tilde{U}_{\bot}^T A\| \|Q_{\tau } \| \| \tilde{\boldsymbol{x}}_1
\|_2 \le \| \tilde{U}_{\bot}^TA \|  \| \tilde{\boldsymbol{x}}_1
\|_2  = \lambda_{K+1}(A) \| \tilde{\boldsymbol{x}}_1\|_2 \le\| (A - M)\| \|\tilde{\boldsymbol{x}}_1\|_2 \cr
\|\tilde{U}^T AQ_{\tau }\tilde{\boldsymbol{x}}_1\|_2 & = \|(\tilde{U}^T
A \tilde{U} \tilde{U}^T Q_{\tau } + \tilde{U}^T A \tilde{U}_\bot
\tilde{U}_{\bot}^T Q_{\tau })\tilde{\boldsymbol{x}}_1\|_2 \cr & \ge  \|\tilde{U}^TA \tilde{U} \tilde{U}^T Q_{\tau }
\tilde{\boldsymbol{x}}_1 \|_2 - \|\tilde{U}^T A \tilde{U}_\bot \tilde{U}_{\bot}^T Q_{\tau }\tilde{\boldsymbol{x}}_1\|_2\cr
& \ge \lambda_K(A) \|\tilde{U}^TQ_{\tau}\tilde{\boldsymbol{x}}_1\|_2 \ge (\lambda_K(M) - \|A-M \| ) \|\tilde{U}^TQ_{\tau}\tilde{\boldsymbol{x}}_1\|\cr 
& \ge (\lambda_K(M) - \|A-M \| ) \sqrt{1- \|\tilde{U}_{\bot}^T
  Q_{\tau} \|_2^2}.
\end{align*}

Let $\zeta = \frac{\|A -M \|_2^2}{(\lambda_K (M) -
  \|A -M \|_2 )^2}$.  Since $\frac{\|A -M
  \|_2}{\lambda_K (M)} = o(1)$, $\zeta= O(\frac{\|A -M \|_2^2}{\lambda_K (M) ^2}) = o(1)$. Then, from \eqref{eq:uqbnd},
$$1-\|\tilde{U}_{\bot}^T Q_{\tau + 1} \|_2^2 \ge 1-\frac{\zeta}{1-\|\tilde{U}_{\bot}^T
  Q_{\tau} \|_2^2 +\zeta} = \frac{1-\|\tilde{U}_{\bot}^T
  Q_{\tau} \|_2^2 }{1-\|\tilde{U}_{\bot}^T
  Q_{\tau} \|_2^2 +\zeta}.$$
When $1-\|\tilde{U}_{\bot}^T  Q_{\tau} \|_2^2 \le \zeta$, $1-\|\tilde{U}_{\bot}^T Q_{\tau + 1} \|_2^2 \ge  \frac{1-\|\tilde{U}_{\bot}^T
  Q_{\tau} \|_2^2 }{2\zeta}.$ From this, one can easily check that when $\tau \ge \frac{\log
  (\zeta/(1-\|\tilde{U}_{\bot}^T Q_{0}\|_2^2))}{\log (1/2 \zeta)}$,
$1-\|\tilde{U}_{\bot}^T  Q_{\tau} \|_2^2 \ge \zeta$,
$1-\|\tilde{U}_{\bot}^T  Q_{\tau+1} \|_2^2 \ge 1/2$, and
$1-\|\tilde{U}_{\bot}^T  Q_{\tau+2} \|_2^2 \ge 1- 2\zeta$.
Therefore, when $\frac{\log |V|}{2} \ge \frac{\log
  (\zeta/(1-\|\tilde{U}_{\bot}^T Q_{0}\|_2^2))}{\log (1/2 \zeta)}$, $\|\tilde{U}_{\bot}^T Q_{\tau^{\star}} \|_2=O\left( \frac{\|A-M \| }{\lambda_K (M)}
\right)$. Since $\zeta = o(1)$, to complete this proof, it is sufficient to show that $1-\|\tilde{U}_{\bot}^T
Q_{0}\|_2^2 \ge 1/x(|V|)$ with probability $1-O(1/|V|)$, where $x(|V|)$
is a polynomial function of $|V|$ with finite
order. By Theorem 1.2 of \cite{rudelson2008} (Please refer
to the proof of Lemma 10 of \cite{mitliagkas2013}) we can conclude this part with $x(|V|)=1/(|V|)^4$.

\noindent\underline{\em ii) $\|U_{\bot}^T\tilde{U}\| = O\left( \frac{\|A-M \| }{\lambda_K (M)}
\right)$:} We can get an upper bound and a lower bound for $\|  A U_{\bot} \|$ as follows:
\begin{align*}
\|  A U_{\bot} \|& = \|  (M + A - M) U_{\bot} \| =
\|  (A - M) U_{\bot} \| \le \|A - M \| \cr
\|  A U_{\bot} \|& = \|  (\tilde{A} + A - \tilde{A}) U_{\bot} \| \ge
\|  \tilde{A}U_{\bot} \|- \|  (A - \tilde{A})
U_{\bot} \|  \ge
\|  \tilde{U} \tilde{\Lambda} \tilde{U}^T U_{\bot} \|- \| A -
\tilde{A} \| \cr & \ge \lambda_{K}(A) \| \tilde{U}^T U_{\bot} \|- \| A
- \tilde{A} \| \ge ( \lambda_{K}(M) - \|A-M\|) \| \tilde{U}^T U_{\bot} \|- \| A - M \| .
\end{align*}
When we combine above bounds, 
$ \| \tilde{U}^T U_{\bot} \| \le \frac{2 \| A - M \|}{ ( \lambda_{K}(M) - \|A-M\|)} =O\left( \frac{\|A-M \| }{\lambda_K (M)}
\right)$.

\subsection{Proof of Lemma~\ref{lem:detection}}\label{sec:proof-lemma-refl-1}
From the definitions of $U_B $ and $U_{\bot}$,
$Q = U_BU_B^T Q + U_{\bot}U_{\bot}^TQ$.
Since rows of $U_B$ corresponding to the nodes from the same cluster
are the same, the rows of $U_BU_B^T Q$ are also the same for the node from
the same clusters. Let $U_BU_B^T Q(k)$ be
the rows of $U_BU_B^T Q$ corresponding to $v\in V_k$. Let
${\boldsymbol v}_{(k \ell)} \in
\mathbb{R}^{K\times 1}$ such that $k$-th row and $\ell$-th row are $1/\sqrt{|V_k|}$ and $-1/\sqrt{|V_\ell|}$,
respectively and other elements  are zero. Then, $\| U_BU_B^T Q(k) - U_BU_B^T Q(\ell)
\|^2 = \| U_B^T Q {\boldsymbol v}_{(k \ell)}\|^2
$.  Since $\|U_B^T Q
\boldsymbol{x} \| \ge 1 - \| U_{\bot}^TQ \|$ for all
$\|\boldsymbol{x}\| =1$, 
$$\| U_BU_B^T Q(k) - U_BU_B^T Q(\ell)
\|^2 = \Omega( \frac{1 - \| U_{\bot}^TQ \|}{|V|} )= \Omega(\frac{1}{|V|}) \quad\mbox{for all}~
k\neq \ell. $$  
Therefore, with some positive $C>0$,
\begin{align*}
C &\frac{ |\bigcup_{k,\ell: k \neq \ell}
  S_k \bigcup V_\ell |}{|V|}  \le \sum_{k,\ell: k \neq \ell}
\sum_{v\in  S_k \bigcup V_\ell} \|U_BU_B^T Q(k) - U_BU_B^T Q(\ell ) \|^2 \cr
& \le 2 \sum_{k,\ell : k \neq \ell}
\sum_{v\in  S_k \bigcup V_\ell} \|U_BU_B^T Q(k) - \xi_{i^{\star},k} \|^2
+\|\xi_{i^{\star},k} - U_BU_B^T Q(\ell ) \|^2 \cr
&\le 4 \sum_{k,\ell : k \neq \ell}
\sum_{v\in  S_k \bigcup V_\ell} \| U_BU_B^T Q(\ell ) - \xi_{i^{\star},k}
\|^2 \cr
&\le 8 \sum_{k,\ell : k \neq \ell}
\sum_{v\in  S_k \bigcup V_\ell} \| U_BU_B^T Q(\ell ) - Q_v
\|^2 + \|  Q_v - \xi_{i^{\star},k} \|^2 \cr
&\le 8  \|U_{\bot}U_{\bot}^TQ\|_F^2 + 8r_{i^{\star}} \le 8 K
\|U_{\bot}U_{\bot}^TQ\|^2 + 8r_{i^{\star}} \le 8 K
\|U_{\bot}^TQ\|^2 + 8r_{i^{\star}}
\end{align*}

To conclude this proof, we need to show that $r_{i^{\star}} =
O(\|U_{\bot}^TQ\|^2)$. Let $i^t$ be an integer between $1$ and $\log
|V|$ such that  $\frac{\|U_{\bot}U_{\bot}^TQ\|_F^2 }{|V|
  \delta^2} \le \frac{i^t}{|V|\log |V|} \le \frac{\delta^2}{|V|}$ with
positive constant
$\delta$ close to 0. There exists such $i^t$ for any $\delta$, since   $\|U_{\bot}U_{\bot}^TQ\|^2 = o(1)$ and the rank of
$U_{\bot}U_{\bot}^TQ$ is $K$. Then, 
\begin{align*}
\Big|\bigcup_{1\le k \le K} \{ v \in V_k : \|Q_v - U_BU_B^T Q(k ) \|^2 \le
\frac{i^t }{4 |V|\log |V|} \} \Big| &\ge |V| -
\|U_{\bot}U_{\bot}^TQ\|_F^2\frac{4 |V|\log |V|}{i^t } \cr
&\ge |V|(1-4\delta^2).\end{align*}
From this, since $\|Q_v - Q_w \|^2 \le 2\|Q_v - U_BU_B^T Q(k )\|^2 + 2\|Q_w -
U_BU_B^T Q(k )\|^2 $, when $v$ satisfying that $\|Q_v - U_BU_B^T Q(k ) \|^2 \le
\frac{i^t}{4 |V|\log |V|},$ $$|W_{i^t,v}| \ge |V_k|- 4\delta^2|V|.$$ On
the other hand, since $\|Q_v - Q_w \|^2 \ge \frac{1}{2}\|Q_v - U_BU_B^T Q(k )\|^2 -\|Q_w -
U_BU_B^T Q(k )\|^2 $, when $v$ satisfying that $\|Q_v - U_BU_B^T Q(k ) \|^2 \ge
\frac{i^t}{ |V|\log |V|},$ $$|W_{i,v}| \le  4\delta^2|V|.$$ With small
enough constant $\delta$, therefore, when $v$ and $w$ satisfy that $\|Q_v - U_BU_B^T Q(k ) \|^2 \le
\frac{i^t}{ |V|\log |V|}$ and $\|Q_w - U_BU_B^T Q(k ) \|^2 \ge
\frac{i^t}{ |V|\log |V|},$ $|W_{i,v}| > |W_{i,w}|$, which indicates
that the origin of $T_{i^t, k}$ is at least $\|Q_{v_k} - U_BU_B^T Q(k ) \|^2 \le
\frac{i^t}{ |V|\log |V|}$ and $|T_{i^t,
, k}| \ge |V_k| - 4\delta^2 |V| $. Since $\|\cdot \|$ is a
convex function, by Jensen's inequality, for all $k$, 
$$\|U_BU_B^T Q(k ) - \xi_{i^t,k}\|^2 \le \frac{\sum_{v \in T_{i^t , k}}
  \|U_BU_B^T Q(k ) - Q_v\|^2 }{|T_{i^t , k}|} \le
\frac{\|U_{\bot}U_{\bot}^TQ\|_F^2 }{|V_k| - 4\delta^2 |V|} =  O(\frac{\|U_{\bot}^TQ\|^2 }{|V|}).$$
Therefore,
\begin{align*}
r_{i^t} & =  \sum_{k=1}^K \sum_{v \in T_{i^t,k}} \|Q_v - \xi_{i^t,k} \|^2  \le \sum_{k=1}^K \sum_{v \in V_k} \|Q_v - \xi_{i^t,k} \|^2 \cr
 &\le 2\sum_{k=1}^K \sum_{v \in V_k } \|Q_v - U_BU_B^T Q(k ) \|^2 +\|U_BU_B^T
 Q(k ) - \xi_{i^t,k} \|^2 \cr
 &\le 2 \|U_{\bot}U_{\bot}^TQ\|_F^2 +2\sum_{k=1}^K \sum_{v \in V_k }
 \|U_BU_B^T Q(k ) - \xi_{i^t,k} \|^2 \cr
& = O ( \|U_{\bot}^TQ\|^2)+2\sum_{k=1}^K \sum_{v \in V_k }
 \|U_BU_B^T Q(k ) - \xi_{i^t,k} \|^2 = O ( \|U_{\bot}^TQ\|^2).
\end{align*}
Since $r_{i^{\star}} \le r_{i^t}$, $r_{i^{\star}} = O ( \|U_{\bot}^TQ\|^2).$



\section{Block-Stochastic power method}
\begin{algorithm}[h!]
   \caption{Block-Stochastic Power method}
   \label{alg:BSPmethod}
\begin{algorithmic}
\STATE {\bfseries Input:} $\{A_1, \dots, A_T \}$, $p$, $K$
\STATE {\bfseries Initial:} $Q_0 \leftarrow$Randomly choose $K$
orthonormal vectors,  $B \leftarrow \frac{g(n) \log n}{p} $, and $\tau^\star \leftarrow \lfloor \frac{T}{B} \rfloor$
\FOR{$\tau=1$ {\bfseries to} $\tau^\star$}
\STATE $S_\tau \leftarrow$ $n\times K$ size zero matrix 
\FOR {$t= 1+(\tau-1)B$ {\bfseries to} $\tau \cdot B$}
\IF{$A_t^T \cdot {\boldsymbol 1} \le 10np$}
\STATE $S_\tau \leftarrow S_\tau + \frac{1}{B}  (A_t A_t^T - \mbox{diag}(A_t A_t^T)) Q_{\tau-1}
$ 
\ENDIF
\ENDFOR 
\STATE $S_\tau = Q_\tau R_{\tau}$
\ENDFOR
\STATE $(\hat{V}_k)_{1\le k \le K}
\leftarrow$Detection$(Q_{\tau^\star} ,V, K)$ 
\STATE {\bfseries Output:} $(\hat{V}_k)_{1\le k \le K}$,
\end{algorithmic}
\end{algorithm}

In this section, we discuss how the schemes developed for streaming PCA could be applied to our problem. We assume here that columns are independent and that we know $p$ ( we are indeed able to estimate $p$ from first few columns by the law of large numbers).

Algorithm~\ref{alg:BSPmethod} presents the Block-Stochastic power method
for SBM, which is an extension of memory limited streaming
PCA \cite{mitliagkas2013}. The eigenvectors corresponding to the $K$ largest
eigenvalues of $M$ contain the community structure. Thus, finding $K$
dimensional structure, the linear span of the eigenvectors (approximately), we can
deduce the communities accurately.

At each time block, we take the product of the empirical covariance matrix for the
length $B$ block and the $K$ orthonormal vectors estimated from the
previous block. If the empirical covariance matrices of all blocks
are close to  $M^2$, the power method amplifies the
principle components which contain the community information. The
matrix Bernstein inequality gives the distance between the
empirical covariance matrices and $M^2$. 
\begin{proposition}[Matrix Bernstein] Consider a finite independent
  random matrix set $\{ X_i \}_{1\le i \le B}$, where every $X_i$ are
  self-adjoint with dimension $n$, $\mathbb{E}[X_i] = 0$,
  $\lambda_{\max} (X_i) \le R$ where $\lambda_{\max}(X)$ is the largest
  eigen value of $X$. Let $\rho^2 = \|\frac{1}{B} \sum_{i=1}^{B}
  \mathbb{E}[X_i^2] \|$. Then,
$$\mathbb{P} \{ \lambda_{\max} (\frac{1}{B}\sum_{i=1}^{B} X_i) \ge x \} \le n
\exp\left(\frac{-B\cdot x^2/2}{\rho^2 + Rx/3} \right).$$
\end{proposition} 
To use the matrix Bernstein inequality, we have to use two tricks:
remove the diagonal of the empirical covariance
matrix since the diagonal term becomes biased, and remove all
arrivals having more than $10np$ positive entries so that 
$\lambda_{\max}(A_i A_i^T)$ and $\rho^2$ can be bounded.
With the tricks, we conclude  Lemma~\ref{lem:normdist} from the matrix Bernstein inequality.
\begin{lemma} When $B = n \log n \frac{g(n)}{f(n)}$, with probability $1-1/n$,
$$ \left\| \frac{1}{B}\sum_{i=1}^B\big(A_i A_i^T -
  \mbox{diag}(A_i A_i^T) \big) -\frac{1}{n} M^2 \right\| = O \left(
    \frac{np^2}{g(n)^{1/2}} \right)  .$$\label{lem:normdist}
\end{lemma}
Then, the
Block-Stochastic power method is approximately the power method by $M^2$.
Therefore, when $\tau^{\star} \ge \log n$, $Q_{\tau^{\star}}$ becomes very close to
the $K$ dimensional principle component of $M$ and thus we can find
the communities accurately from $Q_{\tau^{\star}}$.
\begin{theorem}
When $T \ge n \log^2 n \frac{g(n)}{f(n)}$, with probability 0.99,
$$\frac{1}{n} \left|\bigcup_{1\le k \le K} \hat{V}_k \setminus V_k
\right| = O\left( (g(n))^{-1} \right). $$\label{thm:block-stoch-power}
\end{theorem}
\begin{remark}
Let $T=n$. When $f(n) = \omega (\log^2 n )$, the condition of
Theorem~\ref{thm:block-stoch-power} holds. Therefore, $f(n) =
\Omega(g(n)\log^2 n)$ is the sufficient condition for community detection with one-pass streaming by
Algorithm~\ref{alg:BSPmethod} for given error $O(g(n)^{-1})$. Note that the sufficient condition is $f(n) =
\Omega(\log g(n))$ with Algorithm~3.
\end{remark}


\subsection{Proof of Lemma~\ref{lem:normdist}}
Let $X_i = \big(A_i A_i^T -
  \mbox{diag}(A_i A_i^T) \big) -\frac{1}{n} \big( M^2 -
  \mbox{diag}(M^2 )\big) $. We know that
$\mathbb{E} \left[ X_i  \right] = 0$. Since $A_i^T {\boldsymbol 1}
\le 10np$, 
\begin{align*}\|X_i \| &= \| \big(A_i A_i^T -
  \mbox{diag}(A_i A_i^T) \big) -\frac{1}{n} \big( M^2 -
  \mbox{diag}(M^2 )\big) \|  \cr &\le \| \big(A_i A_i^T -
  \mbox{diag}(A_i A_i^T) \big) \| + \| \frac{1}{n} \big( M^2 -
  \mbox{diag}(M^2 )\big) \| \le 20np.
\end{align*}
Since $\mathbb{E}[(X_i)^2] = \mathbb{E}[(X_j)^2]$ for all $i$ and $j$,  
\begin{align*}
\left\|\frac{1}{B}\sum_{i=1}^B \mathbb{E} \left[ (X_i)^2  \right] \right\| = &\left\| \mathbb{E} \left[ (X_i)^2  \right] \right\|  \le \left\| \mathbb{E} \left[
  \big(A_i A_i^T -  \mbox{diag}(A_i A_i^T) \big)^2  \right] \right\|
\le 10 n^2p^3
\end{align*}
Thus, by the Matrix Bernstein inequality, when $B = \frac{g(n) \log
  n}{p}$ and $c_3^2 \ge 40$,
\begin{align*}
\mathbb{P}\left\{ \left\| \frac{1}{B}\sum_{i=1}^B X_i \right\| \le c_3
  \frac{np^2}{\sqrt{g(n)}}
\right\} & \ge 1-2n \exp \left( \frac{-B c_3^2 n^2 p^4 /
    g(n)}{10n^2p^3 + 20 c_3 n^2 p^3 / \sqrt{g(n)}} \right) \ge 1- \frac{1}{n}.
\end{align*}
Therefore, with probability $1-1/n$,
$$ \left\| \frac{1}{B}\sum_{i=1}^B\big(A_i A_i^T -
  \mbox{diag}(A_i A_i^T) \big) -\frac{1}{n} M^2 \right\| \le  \left\|
  \frac{1}{B}\sum_{i=1}^B X_i \right\| + \|\frac{1}{n} \mbox{diag}(M^2) \|= O \left(
    \frac{np^2}{g(n)^{1/2}} \right)  .$$

\subsection{Proof of Theorem~\ref{thm:block-stoch-power}}

$\lambda_{K}(\frac{1}{n}M^2)=\Omega(np^2)$ and  from
Lemma~\ref{lem:normdist}, with high probability, we can bound the
average covariance matrices for all iterations $\tau$ such that $ \left\| \frac{1}{B}\sum_{i=1}^B\big(A_i A_i^T -
  \mbox{diag}(A_i A_i^T) \big) -\frac{1}{n} M^2 \right\| = O \left(
    \frac{np^2}{g(n)^{1/2}} \right) $. Then, analogously with the
  proof of Theorem 3 of
  \cite{mitliagkas2013}, we can show that, with probability 0.99, $\| U_{\bot}^T Q_{\tau{\star}} \| =O\left(
    \frac{1 }{g(n)^{1/2}} \right)$. From
  Lemma~\ref{lem:detection}, we conclude that
$\left| \bigcup_{k=1}^K \hat{V}_k \setminus V_k \right| = O\left(\frac{1}{g(n)} \right)$.


% \subsection{Proof of Lemma~\ref{lem:QU}} \label{sec:proof-lemma-refl}
% Let $\lambda_K( M + X )$
% be the $K$-th largest eigenvalue. Since $M U_\bot = {\boldsymbol 0}$
% and $Q \Lambda^{\star} Q^T$ reduces space to the linear span of $Q$,
% \begin{eqnarray*}
% \| X\|& = &\| X\| \|U_{\bot} \| ~\ge~ \| X U_{\bot} \| ~ = ~ \| (M+X) U_{\bot} \|  \cr
% & \ge & \| Q \Lambda^{\star} Q^T U_{\bot} \| ~ \ge~ \lambda_K( M + X ) \| Q U_{\bot}^T \|
% \end{eqnarray*}
% Since $\lambda_K( M + X ) \ge \lambda_K (M) - \|X \|$, from the above
% inequality,
% $$\| Q U_{\bot}^T \| \le \frac{\|X \|}{\lambda_K (M) - \|X \|}.$$


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "appendix"
%%% End: 

